Black-Box Certification with Randomized Smoothing: A Functional Optimization Based Framework

Randomized classifiers have been shown to provide a promising approach for achieving certified robustness against adversarial attacks in deep learning. However, most existing methods only leverage Gaussian smoothing noise and only work for $\ell_2$ perturbation. We propose a general framework of adversarial certification with non-Gaussian noise and for more general types of attacks, from a unified functional optimization perspective. Our new framework allows us to identify a key trade-off between accuracy and robustness via designing smoothing distributions, helping to design new families of non-Gaussian smoothing distributions that work more efficiently for different $\ell_p$ settings, including $\ell_1$, $\ell_2$ and $\ell_\infty$ attacks. Our proposed methods achieve better certification results than previous works and provide a new perspective on randomized smoothing certification.

==> tex/orig_method.tex <==
\section{Black-box Certification with Functional Optimization} % not a good name?
\label{sec:black-box}

We start with introducing the background of adversarial certification problem and randomized smoothing method. We then introduce in Section~\ref{sec:certification} our general framework for adversarial certification using non-Gaussian smoothing noises, from a  new \functional optimization perspective. Our framework includes the method of \citet{cohen2019certified, teng2020ell} as special cases, %but is applicable to more general families of non-Gaussian smoothing distributions and more types of attacking beyond $\ell_2$ norm. 
%Our new frame
%  
%Importantly, our new framework 
and reveals a potential trade-off between accuracy and robustness that provides important guidance for  better choices of smoothing distributions in Section~\ref{sec:filling}. 



\subsection{Preliminary Knowledge}
%\paragraph{Randomized Smoothed Classifier} 
\paragraph{Adversarial Certification} 
We consider binary classification of predicting binary labels $y\in \{0,1\}$ from feature vectors $x\in \RR^d$ for simplicity. The extension to multi-class cases is straightforward, and is discussed in Appendix. Assume $\ft \colon \RR^d \to [0,1]$ is a given binary classifier ($\sharp$ means the classifier is \emph{given}), which maps from the input space $\RR^d$ 
to either the class probability in interval $[0,1]$ or the binary labels in $\{0,1\}$. 
%is a binary classifier.
In the robustness certification problem, a testing data point $\xt \in \RR^d$ is given,  
%and an \emph{adversarial set} $\B$, which is a neighorhood 
and one is asked to verify if the classifier outputs the same prediction when we perturb the input $\xt$ arbitrarily in $\B$, a given neighborhood of $\xt$.
Specifically, let $\B$ be a set of possible perturbation vectors, \emph{e.g.}, $\B = \{\d \in \RR^d : \norm{\d}_p \leq r\}$ for $\ell_p$ norm with a radius $r$. 
If the classifier predicts $y = 1$ on $\xt$, i.e. $\ftrue(\xt) > 1/2$, we want to verify if $\ftrue(\xt + \vec\delta) > 1/2$ holds for any $\delta \in \B$. In this paper, we consider the most common adversarial settings, \viz. $\ell_1, \ell_2$ and $\ell_\infty$ attacks.
% two types of attacks, including the $\ell_{2}$ attack $\B_{\ell_2,r}\defeq\left\{ \d:\left\Vert \d\right\Vert _{2}\le r\right\} $, and the $\ell_{\infty}$ attack $\B_{\ell_\infty, r}\defeq\left\{ \d:\left\Vert \d\right\Vert _{\infty}\le r\right\} $. 

\paragraph{Black-box Randomized Smoothing Certification} 
Directly verifying $\ftrue$ heavily relies on the smoothness of $\ftrue$, which has been explored in a series of prior works \citep{lecuyer2018certified, wong2017provable}. 
These methods typically depend on the special structure property (\emph{e.g.}, the use of ReLU units) of $\ftrue$,
and thus can not serve as general purpose algorithms. 
Instead, We are interested in \emph{black-box} verification methods that could work for \emph{arbitrary} classifiers. 
One approach to enable this, as explored in recent works \citep{cohen2019certified, lee2019stratified}, is to replace $\ftrue$ with a smoothed classifier by convovling with Gaussian noise, and verify the \emph{smoothed} classifier.

Specifically, assume $\pizero$ is a smoothing distribution with zero mean and bounded variance, \emph{\emph{e.g.}}, $\pizero = \mathcal N(\vec 0, \sigma^2)$. 
The randomized smoothed
classifier is defined by 
\begin{align*} %\label{equ:fsmooth}
\fpizero(\xtrue) := 
\mathbb{E}_{\z\sim\pi_{\boldsymbol{0}}} \left [ \ftrue(\xtrue +\z) \right], % = \fpizero(\xtrue), 
\end{align*}
which returns the averaged probability of $\x+\z$ under the perturbation of $\z \sim \pi_{\boldsymbol{0}}$.
Assume we replace the original classifier with $\fpizero$, then the goal becomes verifying $\fpizero$ using its inherent smoothness. 
Specifically, if $\fpizero(\xtrue) > 1/2$, we want to verify that $\fpizero(\xtrue + \d) > 1/2 $ for every $\d \in \B$, that is, 
\begin{align}
\label{equ:p02}
\min_{\d \in \B} \fpizero(\x +\d) = 
\min_{\d \in \B} \E_{\z\sim \pizero}[\ftrue(\x+\z+\d)]  > \frac{1}{2}.
\end{align}
% \vspace{-1mm}
In this case, it is sufficient to obtain a 
\emph{guaranteed lower bound} of $\min_{\d \in \B} \fpizero(\x +\d)$ and check if it is larger than $1/2$. 
When $\pizero$ is Gaussian $\normal(\vec 0, ~ \sigma^2)$ and for $\ell_2$ attack,  this problem was studied in  \citet{cohen2019certified}, which shows that a lower bound of 
\begin{align}
\label{equ:phib}
\min_{\z \in \B} 
\E_{\z\sim \pizero}[\ftrue(\x +\z)] 
\geq \Phi(\Phi^{-1}(\fpizero(\x))  - \frac{r}{\sigma}), 
\end{align}
where $\Phi(\cdot)$ is the cumulative density function (CDF) of standard Gaussian distribution, and $\Phi^{-1}(\cdot)$ represents its inverse function. 
The proof of this result in \citet{cohen2019certified} 
uses Neyman-Pearson lemma \citep{li1998some}, while in the following section another derivation we revisit this bound via a functional optimization way.
% drawing an interesting connection between adversarial certification and hypothesis testing. 

Note that the bound in \eqref{equ:phib} is tractable since it only requires to evaluate the smoothed classifier $\fpizero(\x)$ at the original image $\xt$, instead of solving the difficult adversarial optimization over perturbation $\z$ in  \eqref{equ:p02}. In practice, $\fpizero(\x)$ is approximated by Monte Carlo approximation with a non-asymptotic confidence bound. 
% For example, assume $\{\z_i\}$ are i.i.d. samples from $\pizero$ and $\hat f =  \sum_{i=1}^n \ftrue(\xtrue + \z_i)/n$, then with probability $1-2\delta$, we have   $|\fpizero(\x)-\hat f| \leq \sqrt{\log (1/\delta)/({2n})}$ for $\delta <1/2$, using Hoeffding inequality. 
%Note that calculating the lower bound in \eqref{equ:fsmooth} requires to evaluate $$

%is result was obtain in


% \iffalse 
% \paragraph{$\D_+$ Discrepancy} 
% We define the following discrepancy between two measure:
% $$
% \D_+\left(f\Vert g\right) := \int\left(f(\z)-g(\z)\right)_{+}d\z = \int\max\left(f(\z)-g(\z), 0\right)d\z
% $$
% \begin{lemma}
% \label{lemma1_discrepancy}
% $\D_+$ follows the triangle inequality: $\D_+\left(f\Vert g\right) \le \D_+\left(f\Vert h\right) + \D_+\left(h\Vert g\right)$
% \end{lemma}

% \begin{lemma}
% \label{lemma2_discrepancy}
% If $f$ and $g$ are both normalized distributions, then $\D_+\left(f\Vert g\right)$ is equal to the total variation distance: 
% $$\D_+\left(f\Vert g\right)=\mathrm{TV}\left(f\Vert g\right) :=\frac{1}{2}\int|f(\z)-g(\z)| d \z$$
% \end{lemma}
% This discrepancy will be used in this section and
% we defer the proof of these lemmas to appendix \ref{sec:discrepancy}.
% \fi 

%\subsection{Certification via \functional Optimization} 
\subsection{Constrained Adversarial Certification}
\label{sec:certification}

%One approach to the certification problem above is to calculate a \emph{guaranteed lower bound} of $E(\pizero, \ftrue, \B)$ and check if it is larger than $0.5$. 
%The key challenge is that the optimization on $\boldsymbol{\delta}$ is often a challenging non-convex optimization problem.
%A guaranteed lower bound must have a exact worst case $\mu$, which cannot be achieved by most of the optimization methods.
%In other words, directly solving an optimization problem $\min_{\d \in \mathcal{B}} f(\d)$ can only yield an upper bound, instead of \emph{guaranteed} lower bound. 
% with non-asymptotic confidence bound.   
%
%\textcolor{red}{TODO: add some discussion on upper - lower bound way in appendix \ref{sec:bilateral}} 
 %However, since in practice $f$ tends to be a complicated functionand the landscape of optimizing $\d$ is non-convex, there is no guarantee that $\min_{\d\in\mathcal{\B}}\pi_{\boldsymbol{0}}[f_{c}](\x+\d)$ can be exactly computed. 
%A natural idea is to find a lower bound of $\min_{\d\in\mathcal{\B}}\pi_{\boldsymbol{0}}[f_{c}](\x+\d)$  that can be exactly computed. 
%To address the problem, we consider 

We propose a \textbf{constrained adversarial certification (CAC)} framework, which yields a guaranteed lower bound for \eqref{equ:p02} based on constrained \functional optimization. 
The main idea is simple: 
assume $\mathcal F$ is a function class which is known to include $\ftrue$,   
then the following optimization immediately yields a guaranteed lower bound,
\begin{equation}
\begin{split}
 & \min_{\d\in\mathcal{\B}}\fpizero(\x+\d) 
\geq \\
&  \min_{f\in\F} \min_{\d\in\mathcal{\B}}
\bigg \{  f_{\pizero}(\x + \d)
~~\mathrm{s.t.}~~
f_{\pizero}(\x) = \fpizero(\x) 
\bigg\}
,
\label{eq:constrant_opt}
\end{split}
\end{equation}

where we define $f_{\pizero}(\x) = \E_{\z\sim \pizero}[f(\x+\z)]$ for any $f$, and search for the minimum value of $f_{\pizero}(\x+\d)$ %\E_{\pizero}[f(\x+\d)]:= \E_{\z\sim\pizero}[f(\x+\d+\z)]$
for all classifiers in $\mathcal F$ and satisfies $f_{\pizero}(\x) = \fpizero(\x)$. This obviously yields a lower bound once $\ftrue \in \mathcal F$. 
%{\color{red}$\ftrue$ vs. $f$ need to be distinguished}
%where $\ftrue$ is the base classifier (\emph{e.g.} a deep neural network)
%and $f$ is an arbitrary function in the function class $\mathscr {F}$.
%Obviously, 
If $\mathcal {F}$ includes only $\ftrue$,  
then the bound is exact, but is computationally prohibitive due to the difficulty of optimizing $\boldsymbol{\delta}$. 
%When 
The idea is then to choose $\F$ properly 
to incorporate rich information of $\ftrue$, while allowing us to 
calculate the lower bound in \eqref{eq:constrant_opt} computationally tractably.
%still yield  computationally tractable lower bound. 
%be properly in order to yield bounds that are both tight and 
%where $\mathcal{F}$ can be viewed as the function class of $f_{c}$and $\mathcal{H}[\cdot]$ is some \functional that extract certain information ofthe \emph{given} classifier $f^*_{c}$ such that $f$ also holds the information.Notice that if $\mathcal{H}[\cdot]$ provides all information of $f_{c}$, thenthe solution of problem (\ref{eq:constrant_opt}) is exactly the solutionof problem (\ref{eq:certify}). $\mathcal{H}$, $\F$ and $\pi_{\boldsymbol{0}}$need to be properly chosen such that the problem \ref{eq:constrant_opt}is solvable. 
In this paper, we consider the set of all functions bounded in $[0,1]$, that is, 
%the following function class, %which draws connection to \citet{cohen2019certified} as we show in the sequel, 
\begin{align}
\F_{[0,1]} & =\bigg \{f:f(\z)\in[0,1], \forall \z\in \mathbb{R}^d \bigg \}, 
%\cap \bigg\{ [\pi_{\boldsymbol{0}}\conv f](\x) =  [\pi_{\boldsymbol{0}}\conv \ftrue](\x) \bigg\}, 
%\mathcal{H}[f] & =\pi_{\boldsymbol{0}}[f](\x).
\label{equ:f01}
\end{align}
which guarantees to include $\ftrue$ by definition. 
There are other $\mathcal F$ that also yields computationally tractable bounds, including the $L_p$ space $\mathcal F =\{f \colon \norm{f}_{L_p} \leq v\}$, which we leave for future work.

% for which we draw more discussion in \red{Appendix \ref{sec:bilateral}}.  
%where we encode the information that $f$ takes values in $[0,1]$,and also matches with $\ftrue$ (i.e., $[\pi_{\boldsymbol{0}}\conv f](\x) =  [\pi_{\boldsymbol{0}}\conv \ftrue](\x) $). 
%The choice of $\F$ is natural for a classifier with softmax layer. We define  $\mathcal{H}[\cdot]$ so that $\mathcal{H}[f^*_{c}]$ is the score of the randomized smoothed classifier on clean image $\x$.
%For more detailed discussion about the function class, we refer the readers to Appendix.
Denote by $\V(\F, \B)$ the lower bound in \eqref{eq:constrant_opt}. We can rewrite it into the following minimax form using the Lagrangian function, % of \eqref{eq:constrant_opt}, we have 
\begin{equation}
\begin{split}
 & \V(\F,\B) = \min_{f\in\F} \min_{\d\in\B} \max_{\lambda\in\R} L(f, \d, \lambda) \\
 & \triangleq \min_{f\in\F} \min_{\d\in\B} \max_{\lambda\in\R}\bigg\{ f_{\pizero}(\x+\d) -\lambda(f_{\pizero}(\x) - \fpizero(\x)) \bigg\},    
\end{split}
\end{equation}
where $\lambda$ is the Lagrangian multiplier. 
Exchanging the $\min$ and $\max$ yields the following dual form. 
%This yields the following dual form of the bound. % which allows tractable computation. 
%{\color{red}Despite the problem of Equation(\ref{eq:constrant_opt}) is a constraint optimization problem on \functional space and vector space, we show that it can be exactly solved by using idea of Lagrange dual method.}

\begin{theorem} \label{thm:dual}
%Denote by $E(\mathcal F, \B)$ the lower bound in \eqref{eq:constrant_opt}, and 
(\textbf{Dual Form}) Denote by $\pi_\d$ the distribution of $\z +\d$  when $\z \sim \pizero$.  
Assume $\F$ and $\B$ are compact set. 
We have the following dual form of $\V(\F, \B)$ via strong duality: 
%Let $L(f, \d, \lambda)$ be the Lagrangian function of the constraint optimization 
%We have the following lower bound by duality: 
\begin{align}
\V(\F, \B) \ge 
\max_{\lambda\geq0}  & \min_{f\in\F}\min_{\d\in\B}  
L(f, \d, \lambda) \\
= \max_{\lambda\ge 0} & \left\{\lambda \fpizero(\x)-\max_{\d\in\mathcal{\B}}\D_{\F}\left(\text{\ensuremath{\lambda}}\pi_{\0}~\Vert~ \pi_{\d} \right)\right\},
\label{equ:mainlowerbound}
\end{align}
where we define $\D_{\F}\left(\text{\ensuremath{\lambda}}\pi_{\0} ~\Vert~ \pi_{\d} \right)$ as
$$ \max_{f \in \F} \Big \{ \lambda\E_{\z\sim\pizero} [f(\x+\z)] - \E_{\z\sim\pi_{\d}}[f(\x+\z)] \Big\}, 
$$
which measures the difference of $\lambda \pizero$ and $\pi_{\d}$ by seeking the maximum discrepancy of the expectation for $f\in \F$. 
As we show later, the bound in (\ref{equ:mainlowerbound}) is computationally tractable with proper  $(\F, \B, \pizero)$.
%akin to integral probability metric (IPM). 

\end{theorem}

% \paragraph{Remark}
% We will show later that the proposed methods and the cases we study satisfy the condition in part III of the theorem and thus all the lower bounds of the proposed method are tight.

%\paragraph{Solving the Optimization}
%Denote $p_{0}=\fpizero(\xt)$ and notice that $p_{0}$ can be estimated with arbitrary precision by Monte Carlo method if we can sample easily from $\pi_{\boldsymbol{0}}$. We defer the analysis on Monte Carlo approximation to Appendix ~\ref{section:algorithm}.
% and assume we know $p_{0}$ for now.
%We analyze \eqref{eq:constrant_opt} from a primal-dual view.Denote $\pi_{\d}$ as the distribution of $\z+\d$ for simplicity, 
%where $\z\sim\pi_{\boldsymbol{0}}$and thus $[\pi_{\boldsymbol{0}}[\conv f](\x+\d)=[\pi_{\d}\conv f](\x)$.Given an input $\x$, the primal problem
%can be relaxed as below under our choice of $\F$ and $\mathcal{H}$:

\begin{proof} 
First, observe that the constraint in \eqref{eq:constrant_opt} can be equivalently replaced by an inequality constraint $f_{\pizero}(\x) \geq \fpizero(\x)$. 
Therefore, the Lagrangian multiplier can be restricted to be $\lambda \geq 0.$ 
%Denote by $\lambda\geq 0$ %{\color{red} as we use equality constraint, $\lambda\in R^d$}
%the Lagrangian multiplier for the inequality constraint. % in \eqref{eq:constrant_opt}. 
We have 
\begin{align*}
 & \V(\F,\B)\\
 = & \min_{\d\in\mathcal{\B}, f\in\F}\max_{\lambda\ge 0}  \Big\{\E_{\pi_{\d}}f(\x+\z)+ \\
 & \quad\qquad\qquad \quad \lambda\left(\fpizero(\x)- \E_{\pizero}f(\x+\z)\right) \Big\}\\
\ge  & \max_{\lambda\ge 0}\min_{\d\in\mathcal{\B},f\in\F} \Big\{\E_{\pi_{\d}}[f(\x+\z)] +\\
&  \quad\qquad \qquad\quad \lambda\left(\fpizero(\x)-
\E_{\pizero}[f(\x+\z)]\right)\Big\} \\
= & \max_{\lambda\ge 0}\min_{\d\in\mathcal{\B}}
 \Big\{ \lambda\fpizero(\x) ~+ \\
 &  \quad\qquad \quad \min_{f\in\F}
\left \E_{\pi_{\d}}[f(\x+\z)] - 
\lambda \E_{\pizero}[f(\x+\z)] \right) \Big\} \\
= & \max_{\lambda\ge 0}\min_{\d\in\mathcal{\B}}
 \left\{\lambda \fpizero(\x) - \D_\F(\lambda \pizero~\Vert~\pi_{\d})\right\}.
\end{align*}
\vspace{-2mm}

We defer the proof of the strong duality to Appendix due to its intricacy.
\end{proof}

Particularly, when $\F = \F_{[0,1]} :=\{f\colon f(x)\in [0,1], ~x\in \R^d\}$, with straightforward calculation we obtain
\begin{align*}
\D_{\F_{[0,1]}}\left(\text{\ensuremath{\lambda}}\pi_{\0} ~\Vert~ \pi_{\d} \right) =  \int\left(\text{\ensuremath{\lambda}}\pi_{\0}(\z)-\pi_{\d}(\z)\right)_{+}d\z,
\end{align*}

where $(t)_+ = \max(0, t)$. In addition, we have 
$0\leq \D_{\F_{[0,1]}}\left(\text{\ensuremath{\lambda}}\pi_{\0} ~\Vert~ \pi_{\d} \right) \leq \lambda$ for any $\pizero$, $\pi_\d$ and $\lambda >0$. Note that $\D_{\F_{[0,1]}}\left(\text{\ensuremath{\lambda}}\pi_{\0} ~\Vert~ \pi_{\d} \right)$ coincides with the total variation distance between $\pizero$ and $\pi_{\d}$ when $\lambda = 1$. 

To go one step further, suppose that for any $\lambda\ge0$,  we have 
$$\min_{\d\in\B}\min_{f\in\mathcal{F}_{[0,1]}}L\left(f,\d,\lambda\right)=\min_{f\in\mathcal{F}_{[0,1]}}L\left(f,\d^{*},\lambda\right),$$
for some $\d^{*}\in\B$, then our bound $\V\left(\mathcal{F},\B\right)$ becomes 
\[\max_{\lambda\ge0}\Big\{\lambda \fpizero(\x) - \int\big(\text{\ensuremath{\lambda}}\pi_{\0}(\z)-\pi_{\d^*}(\z)\big)_{+}d\z\Big\}. \]

% \red{repeat with later section about computation?}
Although the lower bound in  \eqref{equ:mainlowerbound} still involves an optimization on $\vv\delta$ and $\lambda$, 
both of them are much easier than the original adversarial optimization in Equation (\ref{equ:p02}).
With proper choices of $\F$, $\B$ and $\pi_\0$, the optimization of $\vv\delta$ can be shown to provide simple closed form solutions by exploiting the symmetry of $\mathcal B$, 
and the optimization of $\lambda$ is a very simple one-dimensional searching problem.

As corollaries of Theorem \ref{thm:dual}, we can exactly recover the bound derived by \citet{teng2020ell} and \citet{cohen2019certified}.

\begin{corollary}
With Laplacian noise $\pizero(\cdot) = \laplace(\cdot; b)$, where $\laplace(\boldsymbol{x}; b) = \frac{1}{(2b)^d}\exp(-\frac{\Vert\boldsymbol{x}\Vert}{b})$ and $\ell_1$ adversarial setting $\B = \{\d\colon \norm{\d}_{1}\leq r\}$ and $\F =\F_{[0,1]}$, the lower bound in \eqref{equ:mainlowerbound} becomes
\begin{equation}
\begin{split}
\label{equ:resultjiaye}
 &\max_{\lambda \ge 0} \left\{ \lambda \fpizero(\x) -\max_{\|\d\|_1\le r} \D_{\F_{[0,1]}}\left(\text{\ensuremath{\lambda}}\pi_{\0} \Vert \pi_{\d}\right) \right\}\\
= & \left\{  \begin{array}{cc}
             1 -  e^{r/b}(1 - \fpizero(\x)), &\text{when}\quad \fpizero(\x) \geq 1 - \frac{1}{2}e^{-r/b}\\
             &\\
             \frac{1}{2}e^{-\frac{r}{b}-\log[2(1-\fpizero(\x)]}, &\text{when}\quad \fpizero(\x) < 1 - \frac{1}{2}e^{-r/b}
             \end{array}
\right.
\end{split}
\end{equation}
\end{corollary}

\vspace{-4mm}
Thus, with our previous explanation, 
$$
\V(\F,\B)\geq\frac{1}{2} \Longleftrightarrow r \le -b\log\left[2(1 - \fpizero(\x))\right]
$$ 
which is exactly the $\ell_1$ certification radius from \citet{teng2020ell}. 

\begin{corollary}\label{thm:cohen}
With isotropic Gaussian noise $\pizero = \normal(\vv 0, \sigma^2 I_{d\times d})$, 
$\ell_2$ attack $\B = \{\d \colon ~  \norm{\d}_{2}\leq r\}$ and $\F =\F_{[0,1]}$, the lower bound in \eqref{equ:mainlowerbound} becomes
%Solving the optimization
\begin{equation}
\begin{split}
\label{equ:resultCohen}
 &\max_{\lambda \ge 0} \left\{ \lambda \fpizero(\x) -\max_{\|\d\|_2\le r} \D_{\F_{[0,1]}}\left(\text{\ensuremath{\lambda}}\pi_{\0} \Vert \pi_{\d}\right) \right\}\\
= & \Phi\left(\Phi^{-1}(\fpizero(\x))  - \frac{r}{\sigma}\right).
\end{split}
\end{equation}
\end{corollary} 

Analogously, we can retrieve the main theoretical result of \citet{cohen2019certified}:
$$
\V(\F,\B)\geq\frac{1}{2} \Longleftrightarrow r \le \sigma \Phi^{-1}(\fpizero(\x))
$$ 
We defer the corollary proof details to the Appendix.

% \begin{wrapfigure}{r}{0.2\textwidth}
% % \vspace{-15pt}
% %\includegraphics[width=.25\textwidth]{fig/l2_example.pdf} 
% \includegraphics[width=.175\textwidth]{fig/adv.pdf} 
% % \vspace{-10pt}
% % \vspace{-20pt}
% \label{fig:l2_example}
% \end{wrapfigure}

% One key step of the proof is to show that $\max_{\|\d\|_p\le r} \D_{\F_{[0,1]}} \left(\text{\ensuremath{\lambda}}\pi_{\0} \Vert \pi_{\d}\right)$ $p=1, 2$ is achieved when $\d$ is on the boundary of the $\ell_p$ ball $\mathcal B=\{\norm{\d}_p \leq r\}$, which can be, for example, $\d = [r,0,\ldots, 0]^\top$, due to symmetry of $\B$ (see figure on the right for $\ell_2$ case).  \red{zhe duan ting duo yu de}


\subsection{Trade-off between Accuracy and Robustness}
The lower bound in \eqref{equ:mainlowerbound} reflects an intuitive  trade-off between the robustness and accuracy,
\begin{equation}
\label{eq:objective2}
\max_{\lambda \geq 0}\Bigg [ \lambda\underset{\mathrm{Accuracy}}{\underbrace{ \fpizero(\x)}}-\underset{\mathrm{Robustness}}{\underbrace{
\max_{\d\in\B}\D_\F\left(\text{\ensuremath{\lambda}}\pi_{\0}~\Vert~ \pi_{\d} \right)}} \Bigg ], 
\end{equation}
where the first term reflects the accuracy of the smoothed classifier (assuming the true label is $y=1$), 
while the second term $\max_{\d\in\B}\D_\F\left(\text{\ensuremath{\lambda}}\pi_{\0}~\Vert~ \pi_{\d} \right)$  %in \eqref{eq:objective}
measures the robustness of the smoothing method, via the maximum difference between the original smoothing distribution $\pi_\0$ and perturbed distribution $\pi_{\d}$ for $\d\in \B$. The maximization of dual coefficient $\lambda$ can be viewed as looking for a best balance between these two terms to achieve the largest  lower bound. 
%and hence reflect the robustness of the model; 
%Once the distance is smaller,the model can be more robust.
%on the other hand, the first term $ \lambda \fpizero(\x)}$ represents the accuracy.  %assuming the original . %Once you choose a distribution which is not concentrated to the center, the accuracy will be as poor as possible.
%However, if a concentrated distribution is chosen, the distance between the two distributions should be large.

%As shown in \eqref{eq:objective2},
More critically, 
different choices of smoothing distributions  
also yields a trade-off between accuracy and robustness in \eqref{eq:objective2}. 
% If $\pizero$ has large variance or large kurtosis, the distance $\D_\F(\lambda \pizero~\Vert~\pi_{\d})$ will tend to be small thus the smoothed model is robust. 
% However, if the variance of $\pizero$ is too large, we may obtain a low value of $\fpizero(\xt)$ and hence less accurate model. 
The optimal choice of the smoothing distribution should optimally  balance the accuracy and robustness, by distribute its mass properly to yield small $\max_{\d\in\B}\D_\F(\lambda \pizero~\Vert~\pi_{\d})$ and large $\fpizero(\x)$ simultaneously. 
%the samples while not change the distance between $\pi_{0}$ and $\pi_{\d}$ a lot.
% {\color{red} Todo: one figure here?}



% \subsection{A dual perspective of certification}

% % \subsubsection{Retrieving \citet{cohen2019certified}'s bound}
% \subsubsection{Retrieving Cohen's bound}
% % will write this part soon --narsil

% \begin{theorem}[](informal) Solving the \functional optimization
% \begin{align}
%     &\min_{\|\mu\|_2\le r}\min_{0\le f\le1}\mathbb{E}_{\pi_\mu}[f]\\
%     \mathrm{s.t.}\quad & \mathbb{E}_{\pi_{0}}[f]\ge p_0 :=\mathbb{E}_{\pi_{0}}[f^*]
% \end{align}
% can retrieve the bound in \citep{cohen2019certified}, which is $r \ge \sigma \Phi^{-1}(p_0)$
% \end{theorem}

% {This proof will be moved to appendix later.}
% \begin{proof}
% We need to deal with
% $$
% \max_{\lambda \ge 0}
% \min_{\|\mu\|_2\le r}
% &\left\{-\int  \left(\lambda \pizero(z)-
% \pi_{\mu}(z)\right)_{+} d z 
% +  \lambda p \right\}.
% $$
% Define $C_\lambda = \{z: \lambda \pizero(z)\ge
% \pi_{\mu}(z)\} = \{z: \mu^\top z \le \frac{\|\mu\|^2}{2} + \sigma^2\ln\lambda\}$, then
% \begin{align}
%     &\int \left(\lambda \pizero(z)- \pi_{\mu}(z)\right)_{+} d z \\
%     =& \int_{C_\lambda}   \left(\lambda \pizero(z)- \pi_{\mu}(z)\right) d z \\
%     =& \lambda\cdot\mathbb{P}\left(N(z;\boldsymbol{0}, \sigma^2  \mI)\in C_\lambda\right) - \mathbb{P}\left(N(z;\boldsymbol{\mu}, \sigma^2  \mI)\in C_\lambda\right) \\
%     =& \lambda\cdot \Phi\left(\frac{\|\mu\|_2}{2\sigma}+\frac{\sigma\ln\lambda}{\|\mu\|_2}\right) - \Phi\left(\frac{-\|\mu\|_2}{2\sigma}+\frac{\sigma\ln\lambda}{\|\mu\|_2}\right).
% \end{align}
% Let $F(\mu, \lambda) := \lambda p_0 - \int \left(\lambda \pizero(z)- \pi_{\mu}(z)\right)_{+} d z = \lambda p_0 - \lambda\cdot \Phi\left(\frac{\|\mu\|_2}{2\sigma}+\frac{\sigma\ln\lambda}{\|\mu\|_2}\right) + \Phi\left(\frac{-\|\mu\|_2}{2\sigma}+\frac{\sigma\ln\lambda}{\|\mu\|_2}\right)$

% \end{proof}
\section{Improving Certification Bounds with New Distribution Family}%Centripetal distribution: a new distribution family for better certification}
\label{sec:filling}

In this section, we identify a key problem of using Laplacian and Gaussian noise in high dimensional space, due to the ``thin shell'' phenomenon that the probability mass of Gaussian distributions  concentrates on a sphere far away from the center points under high dimensional settings~\citep{vershynin2018high}. Motivated by this observation, we propose a new family of smoothing distributions that alleviate this problem for $\ell_1$, $\ell_2$ and $\ell_\infty$ attack.

\subsection{$\ell_2$ Region Certification} \label{sec:L2}

Although isotropic Gaussian distributions appears to be a natural choice of smoothing distributions, 
they are in fact sub-optimal for trading-off accuracy and robustness in \eqref{eq:objective2}, especially in high dimensions. 
%Gaussian distributions seems natural for noising and possesses nice mathematical properties. However, there lies a curse of dimensionality. 
The key problem is that, in high dimensional spaces, 
the probability mass of Gaussian distributions
concentrates on a \emph{thin shell} away from the center.
%Specifically, 

\begin{lemma}
[% Concentration of Norm 
%\emph{Thin Shell} bound
\citet{vershynin2018high}, Section~3.1]
%\red{TODO, find a easier version}
Let $\z \sim  \normal(\vec 0, ~ I_{d\times d})$ be a $d$-dimensional standard Gaussian random variable. Then there exists a constant $c$, such that for $\delta \in (0,1)$,  
$\mathrm{Prob}$ $\left ( \sqrt{d} - \sqrt{c\log(2/\delta)} \leq \norm{\z}_2 \leq \sqrt{d} +  \sqrt{c\log(2/\delta)} \right) \geq 1-\delta.  %1-4\exp(-c^2/4)/c^2. 
$
%$$\mathrm{Prob}( \sqrt{d-1} - c \leq \norm{z}_2 \leq \sqrt{d-1} + c) \geq 1-4\exp(-c^2/4)/c^2. $$
This suggests that with high probability,
$\z$ takes values very close to the sphere of radius $\sqrt{d}$, within a constant distance from that sphere! 
See \citet{vershynin2018high} for more discussion. 
\end{lemma}
%(Deviation). Theorem 3.1.1 states

%Such small, constant deviations could be surprising at the first sight, so let us
%explain this intuitively. The square of the norm, Sn := kXk22 has mean n andstandard deviation O(√n). (Why?) Thus kXk2 =√Sn ought to deviate by O(1)around √n. This is because
%
%
This phenomenon makes it problematic to use standard Gaussian distribution for adversarial certification, 
because one would expect that the smoothing distribution should concentrate around the center (the original image) 
in order to make the smoothed classifier close to the original classifier (and hence accurate). 
To illustrate the problem, 
consider a simple example when the true classifier is $\ftrue(\vv x) = \mathbb{I}(\norm{\vv x - \x}_2\leq \epsilon\sqrt{d})$ for a constant $\epsilon <1$, where $\mathbb{I}$ is the indicator function.  
Then when the dimension $d$ is large, we would have $\ftrue(\x) = 1$ while $\fpizero(\x) \approx 0$ when 
$\pizero = \normal(\vec 0, I_{d\times d})$. 
It is of course possible to decrease the variance of $\pizero$ to improve the accuracy of the smoothed classifier $\fpizero$. However, this would significantly improve the distance term in \eqref{eq:objective2} and does not yield an optimal trade-off on accuracy and robustness.

%For instance, if $X=(X_1, \cdots, X_d)$ is a random variable with distribution $N(\0, \sigma^2 \boldsymbol{I}_d)$, then the expectation of the square of its euclidean distance to zero point has the following property:
%$$\mathbb{E}\left[\|X\|_2^2\right]/d =  \mathbb{E}\left[\frac{\sum_{i=1}^d X_i^2}{d}\right] \stackrel{d\to \infty}{\longrightarrow} \sigma^2.$$
%This shows that when the dimension $d$ is large, the samples of an isotropic Gaussian will concentrate to a very thin spherical "shell" with radius $\sqrt{d}\cdot\sigma$, which is quite far from the center as the norm is proportion to $\sqrt{d}$. This will restrict the performance when estimating $p_0$ as the samples $x+z$ are actually far from the original image $x$. Intuitively, we should modify our distribution to force its mode to be near zero.

In this work, we introduce a new family of distributions to address this curse of dimensionality. To motivate our method, it is useful to examine the density function of the distributions of the radius of spherical distributions in general. 

\begin{lemma} 
 Assume $\z$ is a spherically symmetric random variable on $\R^d$ with a 
%Assume the 
probability density function (PDF) of form $\pizero(\z)\propto \phi(\norm{\z})$, where $\phi \colon [0,\infty) \to [0,\infty)$ is a univariate function, then the PDF of the norm of $\z$ is $p_{\norm{\z}}(r) \propto r^{d-1} \phi(r)$.   The term $r^{d-1}$ arises due to the integration on the sphere of radius $r$ in $\RR^d$. 
\end{lemma}

In particular, when $\z \sim \normal(0, \sigma^2 I_{d\times d})$, 
we have $\phi(r) = \exp(-r^2/(2\sigma^2))$ and hence 
$p_{\norm{\z}_2}(r) \propto r^{d-1}\exp(-r^2/(2\sigma^2))$, which is a scaled Chi distribution, also known as Nakagami distribution. 
Examining this \emph{PDF},  
we can see that the concentration of the norm is caused by the  $r^{d-1}$ term, which makes the density to be highly peaked when $d$ is large.  
To alleviate the concentration phenomenon, 
we need to have a way to cancel out the effect of $r^{d-1}$. This motivates the following family of smoothing distributions: 
\begin{equation}
    \begin{split}
        & \pi_{\boldsymbol{0}}(\z)
        \propto\left\Vert \z\right\Vert _{2}^{-k}\exp\left(-\frac{\left\Vert \z\right\Vert _{2}^{2}}{2\sigma^{2}}\right), \\
        & \text{and hence}
        p_{\norm{\z}_2}(r)\propto r^{d-k-1} \exp\left (-\frac{r^2}{2\sigma^2} \right), 
    \label{equ:L2smooth}
    \end{split}
\end{equation} 
where we introduce a $\left\Vert \z\right\Vert _{2}^{-k}$ term in $\pizero$, with $k$ a positive parameter, to make the radius distribution less concentrated when $k$ is large. 
%when $p$ denotes the $\ell_p$ norm, $\sigma_r$ denotes the variance of the radius (which is similar to the variance of Gaussian distribution) and $k$ controls the concentration to the mean. 

\begin{figure} % {r}{0.35\textwidth}  
% \vspace{-10pt}
\begin{tabular}{c}
     \raisebox{5.5em}{\rotatebox{90}{Variance}} 
     \includegraphics[width=0.4\textwidth]{fig/gamma_mean_variance_modify.pdf} \\
     {Mean}\\
\end{tabular}
\vspace{-10pt}
\caption{\small Starting from radius distribution in \eqref{equ:L2smooth} with $d=100$ $\sigma=1$ and $k=0$ (black start),  
increasing $k$ (green curve) allows us to move the mean towards zero \emph{without
significantly reducing the variance}. 
%In constrast, 
Decreasing $\sigma$ (red curve) can also decrease the mean, but with a cost of decreasing the variance quadratically.  
% \red{Add a legend: ("green": increasing $k$, "red": decreasing $\sigma$)}
%allows us to decrease mean 
%adjust
}
\label{fig:meanvariance}
\end{figure}

The radius distribution in \eqref{equ:L2smooth} is controlled by two parameters $(\sigma, ~ k)$, where $\sigma$ controls the scale of the distribution (and is hence the \emph{scale parameter}), while $k$ controls the shape of the distribution (and hence the \emph{shape parameter}). 
The key idea is that adjusting $k$ allows us to trade-off the accuracy and robustness much more optimally. 
%
As shown in Figure~\ref{fig:meanvariance}, adjusting $\sigma$ 
% \vspace{-3mm} 
enables us to move the mean close to zero (hence yielding higher accuracy), 
but at cost of decreasing the variance quadratically (hence more less robust). In contrast, adjusting $k$ allows us to decrease  the mean without significantly impacting the variance, and hence yield a much better trade-off on the accuracy and robustness. % much more optimally.   




\iffalse 
\begin{figure}
\centering
% \setlength{\tabcolsep}{2em}
\vspace{-30pt}
\begin{tabular}{cc}
% \raisebox{0.5em}{\rotatebox{90}{\small Log [Accuracy (\%)] }} 
\includegraphics[width=0.45\textwidth]{fig/change_sigma_mark.pdf} & \includegraphics[width=0.45\textwidth]{fig/change_k_mark.pdf} \\
\vspace{-0pt}
\vspace{-1\baselineskip}
\large $\|\boldsymbol{x}\|_2$ & \large $\|\boldsymbol{x}\|_2$\\
\end{tabular}
\caption{ This figure shows the empirical distribution for the radius ($\|\boldsymbol{x}\|_2$). 
Changing $\sigma$ will change not only the mean but also the variance.
On the other hand, 
changing $k$ will influence the mean, but have little impact on the variance.
}
\label{fig:l2_example}
\end{figure}
\fi 


\paragraph{Computational Method}  
With the more general non-Gaussian smoothing distribution, we  no longer have the closed form solution of the bound like \eqref{equ:resultCohen}. However, efficient computational methods can be still developed for calculating the bound in  \eqref{equ:mainlowerbound} with $\pizero$ in \eqref{equ:L2smooth}. The key is that %distance term 
the maximum of the distance term 
 $\D_{\F_{[0,1]}}(\lambda \pizero~||~ \pi_{\d})$ over $\d\in \B$ 
 is always achieved on the boundary of $\B$ as we show in the sequel, 
 %and 
 %, %yields a simple closed form 
 %due to symmetry, and 
 while the optimization on $\lambda\geq 0$ is one-dimensional and can be solved numerically efficiently. %because it is an . 
%it can still 

\begin{theorem} \label{thm:opt_mu_l2}
Consider the $\ell_{2}$ attack with $\boldsymbol{\mathcal{B}}=\left\{ \d:\left\Vert \d\right\Vert  _{2}\le r\right\}$ and smoothing distribution  $\pi_{\0}(\z)\propto\left\Vert \z\right\Vert _{2}^{-k}\exp\left(-\frac{\left\Vert \z\right\Vert _{2}^{2}}{2\sigma^{2}}\right)$ with $k\ge0$ and $\sigma>0$.  
Define $\d^{*} = [r,0,...,0]^\top$, we have 
$$
\mathbb{D}_{\mathcal{F}_{[0,1]}}\left(\lambda\pi_{\0}~\Vert~\pi_{\d^*}\right) = \max_{\delta\in\B}\mathbb{D}_{\mathcal{F}_{[0,1]}}\left(\lambda\pi_{\0}~\Vert~\pi_{\d}\right). 
$$
%where 
\end{theorem}
%

With Theorem~\ref{thm:opt_mu_l2},
we can compute \eqref{equ:mainlowerbound} with $\d = \d^*$. We then calculate $\mathbb{D}_{\mathcal{F}_{[0,1]}}\left(\lambda\pi_{\0}~\Vert~\pi_{\d^*}\right)$ using Monte Carlo approximation. Note that 
$$
\mathbb{D}_{\mathcal{F}_{[0,1]}}\left(\lambda\pi_{\0}~\Vert~\pi_{\d^*}\right)
% = \int\left(\text{\ensuremath{\lambda}}\pi_{\0}(\z)-\pi_{\d^*}(\z)\right)_{+}d\z
= \E_{\z\sim \pizero}\left [\left (\lambda-\frac{\pi_{\d^*}(\z)}{\pizero(\z)}\right )_+\right ],
$$
which can be approximated with Monte Carlo method with Hoeffding concentration bound. 
Let $\{\z_{i}\}_{i=1}^n$ be an i.i.d. sample from $\pizero$, then we can approximate 
$\mathbb{D}_{\mathcal{F}_{[0,1]}}\left(\lambda\pi_{\0}~\Vert~\pi_{\d^*}\right)$ with $\hat D := n^{-1}\sum_{i=1}^n \left (\lambda-{\pi_{\d^*}(\z_i)}/{\pizero(\z_i)}\right )_+$. Because $0 \leq \left (\lambda-{\pi_{\d^*}(\z_i)}/{\pizero(\z_i)}\right )_+\leq \lambda$, we have 
$
\mathbb{D}_{\mathcal{F}_{[0,1]}}\left(\lambda\pi_{\0}~\Vert~\pi_{\d^*}\right) \in [\hat D - \lambda\sqrt{\log(2/\delta)/({2n})}, \hat D+ \lambda\sqrt{\log(2/\delta)/({2n})}]
$ with probability $1-\delta$ for $\delta \in (0,1)$. 
Drawing sufficiently large number of samples allows us to achieve approximation with arbitrary accuracy. 
% Finally, the optimization of $\lambda$ in \eqref{equ:mainlowerbound}can be solved numerically with gradient descent.

%\paragraph{$\ell_2$ Region Certification}
%For $\ell_2$ region certification, the distribution is:
% To illustrate the two component of centripetal distribution, one can see our choice for $\ell_2$ case:
%$$\pi_{\boldsymbol{0}}(\z)&\propto\left\Vert \z\right\Vert _{2}^{-k}\exp\left(-\frac{\left\Vert \z\right\Vert _{2}^{2}}{2\sigma_r^{2}}\right).
%$$
% for some $k \ge0$ and $\sigma_r>0$ in our practice.
%As shown in Figure \ref{fig:l2_example}, when $k = 0$, it will degenerate to an isotropic Gaussian distribution. When $k >0$, which is the general case, the mode of the centripetal distribution will be drawn to the center as $\rho\left(\left\Vert \z\right\Vert\right) = \left\Vert \z\right\Vert _{2}^{-k}$ grows rapidly towards $\0$. 


%A near-zero mode can boost the value of $p_0$,while the second term in \eqref{eq:objective2} will not be much worse when the $\pi_\0$ has a heavy tail.As shown in Figure \ref{fig:l2_example},our proposed distribution can concentrate some samples to $\bf{0}$ with little impact on the tail.On the other hand, simply modifying $\sigma$ will influence not only the mean of $\|\boldsymbol{x}\|_2$, but also the variance as well. Other approached, \emph{e.g.}mixture distribution, cannot trivially achieve similar impact.
% {\color{red} maybe put compare inf.pdf here} some more explain 


%We also prove the location for the worst case $\d$ under the proposed distribution, which means we can solve the optimization of $\d$ analytically and lead to a guaranteed lower bound.

\subsection{$\ell_\infty$ Region Certification}\label{sec:Linfty} 

Going beyond the $\ell_2$ attack, we consider the $\ell_\infty$ attack, whose attacking region is $\B_{\ell_\infty, r}=\{\d \colon \norm{\d}_\infty \leq r\}$. This is a far more difficult problem, because the $\ell_\infty$ ball is substantially larger than the $\ell_2$ ball of the same radius in high dimensional space.
This makes the Gaussian smoothing distribution, as well as our $\ell_2$-based smoothing distribution in \eqref{equ:L2smooth}, unsuitable for $\ell_\infty$ attack. In fact, as shown in the following negative result, if we use \eqref{equ:L2smooth} as the smoothing distribution for $\ell_\infty$ attack, the bound we obtain is effectively the bound we would get for verifying a $\ell_2$ ball with radius $\sqrt{d} r$, which is too large to give meaningful results when the dimension is high. 
%First of all, we can get a naive $\ell_\infty$ certification result with the following statement:
% {\color{red}
\begin{theorem}
With the smoothing distribution $\pizero$ in \eqref{equ:L2smooth}
%of  $\pi_{\0}(\z)\propto \norm{\z}_{2}^{-k}
%\exp\left(-\frac{\left\Vert \z\right\Vert _{2}^{2}}{2\sigma^{2}}\right)$, 
for $\for k\ge0, \sigma>0$,  and $\F = \F_{[0,1]}$ shown in \eqref{equ:f01}, 
the bound we get for  
certifying the $\ell_{\infty}$ attack on  $\B_{\ell_\infty, r}=\{\d:\left\Vert \d\right\Vert _{\infty}\le r\}$ is equivalent 
to that for certifying the $\ell_{2}$ attack on $\B_{
\ell_2, \sqrt{d}r}=\{\d:\left\Vert  \d\right\Vert _{2}\le {\sqrt{d}}r\}$, that is, 
$$
\V(\F_{[0,1]}, ~ \B_{\ell_\infty, r}) = 
\V(\F_{[0,1]}, ~ \B_{\ell_2, \sqrt{d} r}). 
$$
\end{theorem}
% }

% \begin{wrapfigure}{r}{0.22\textwidth}
% \vspace{-30pt}
% \includegraphics[width=.22\textwidth]{fig/linf_space.pdf}
% \vspace{-9pt}
% \caption{\small %Illustration of 
% $\ell_\infty$ and $\ell_2$ balls in high dimension.}
% \label{fig:linftyCool}
% \vspace{-20pt}
% \end{wrapfigure}

The key reason of this negative result is that the furthest points to the origin (vertexes) in $\B_{\ell_\infty, r}$ have an $\ell_2$ radius of $\sqrt{d}r$, illustrated as the ``pointy'' points in Figure~\ref{fig:linftyCool}. %the right. 
Thus, the maximum distance $\max_{\d \in \B_{\ell_\infty, r}} \D_\F(\lambda \pizero~\Vert~ \pi_{\d})$ is achieved at  one of these pointy points, making it equivalent to optimizing in the $\ell_2$ ball with radius $\sqrt{d}r.$ 

In order to address this problem, 
we propose the following new \emph{mixed norm} family of smoothing distribution that uses a mix of $\ell_2$ and $\ell_\infty$ norms:
\begin{align}
\pizero(\z) \propto \norm{\z}_{\infty}^{-k} \exp\left (- \frac{\norm{\z}_2^2}{2\sigma^2} \right ), 
\label{equ:mixednormfamily}
\end{align}
in which we replace the $\norm{\z}_2^{-k}$ term in \eqref{equ:L2smooth} with $\norm{\z}_\infty^{-k}$. 
The motivation is that this allows us to allocate more probability  mass along the ``pointy'' directions with larger $\ell_\infty$ norm, and hence decrease the maximum distance term $\max_{\d \in \B_{\ell_\infty, r}} \D_\F(\lambda \pizero~\Vert~ \pi_{\d})$. 
See Figure~\ref{fig:linftyCool} for an illustration.
% \red{ref incorrect, fix}. 
In practice, we find that this {mixed norm} smoothing distribution in 
 \eqref{equ:mixednormfamily} work much more efficiently than the $\ell_2$ norm-based family in \eqref{equ:L2smooth}. 
%$\B_{\ell_2, \sqr}$
%\mathcal B_{}$
%This suggests a curse of dimensionality for $\ell_\infty$ attack
%But this is far from satisfactory due to the curse of dimensionality. To alleviate this problem, 
% \paragraph{Motivation: \red{TODO}}

%one would naturally think of using
Given the difference of $\ell_2$ and $\ell_\infty$ norms, 
it is also natural to consider the following 
%class of smoothing distributions worth consideration 
 \emph{pure $\ell_\infty$ norm} distributions,  which uses $\ell_\infty$ norm in  both of the terms of the distribution, 
\begin{equation}
\label{eq:inf_inf_distribution}
\pi_{\boldsymbol{0}}(\z)& \propto  \left\Vert \z\right\Vert _{\infty}^{-k}\exp\left(-\frac{\left\Vert \z\right\Vert _{\infty}^{2}}{2\sigma^{2}}\right).
\end{equation}
Unfortunately, this seemingly natural choice does not work  efficiently for $\ell_\infty$ attacks (even worse than the $\ell_2$ family \eqref{equ:L2smooth}).  
This is because the volume of the $\ell_\infty$ ball is in some sense ``too large'' (\emph{e.g.}, compared with the volume of $\ell_2$ ball). 
As a result, in order to make the probability mass of  \eqref{eq:inf_inf_distribution} in a reasonable scale, one has to choose a very small value of $\sigma$, which makes maximum distance term too large to be practically useful. 
%based on previous results under the $\ell_\infty$ setting.
%However, we have the following proposition:
\begin{theorem} \label{thm: impossible linf}
%Consider a $\ell_{\infty}$ perturbation with 
Consider the adversarial attacks on the $\ell_\infty$ ball 
$\B_{\ell_\infty, r}=\{\d:\left\Vert \d\right\Vert _{\infty}\le r\}$.
Suppose we use the smoothing distribution $\pizero$ in \eqref{eq:inf_inf_distribution} and 
%$\pi_{\0}(\z)\propto\left\Vert \z\right\Vert _{\infty}^{-k}\exp\left(-\frac{\left\Vert \z\right\Vert _{\infty}^{2}}{2\sigma^{2}}\right)$
choose the parameters $(k, \sigma)$ such that

1) $\norm{\z}_\infty$  is stochastic bounded when $\z\sim \pizero$, in that for any $\epsilon >0$, there exists a finite $M>0$ such that $\mathrm{P}_{\pizero}(|\z|>M ) \leq \epsilon$;   

2) the mode of $\norm{\z}_\infty$ under $\pizero$ equals $C r$, where $C$ is some fixed positive constant, 
%$\mathcal{O}(1)$ constant. 

%$\mathrm{mode}(\left\Vert \z\right\Vert _{\infty})=Cr$, $\left\Vert \z\right\Vert _{\infty}=\mathcal{O}_{p}(1)$, where $C$
%is some $\mathcal{O}(1)$ constant, 
then for {any $\epsilon\in(0,1)$ and sufficiently large dimension $d$, there exists a constant $t > 1$, such that }, we have 
\[
\max_{\d\in \B_{\ell_\infty, r}}\bigg\{ \mathbb{D}_{\mathcal{F}_{[0,1]}}\left(\lambda\pi_{\0}\parallel\pi_{\d }\right)\bigg\}\ge
(1-\epsilon)\left(\lambda-\mathcal{O}(t^{-d})\right).%\left(1-\frac{0.55}{e^{2}}\right)\left(\lambda-\mathcal{O}(t^{-d})\right),
%
\]
This shows that, in very high dimensions, 
the maximum distance term is arbitrarily close to $\lambda$ 
%in when the dimension $d$ is high is very close to $\lambda$,
which is 
%where $t \in (1,\infty)$ is some constant independent with the dimension $d$. 
%This shows that Note that 
the maximum possible value of  $\mathbb{D}_{\mathcal{F}_{[0,1]}}\left(\lambda\pi_{\0}\parallel\pi_{\d }\right)$ (see Theorem~\ref{thm:dual}). 
{
% \color{red}
In particular, this implies that in high dimensional scenario, once $\ff(\x)\le(1-\epsilon)$ for some small $\epsilon$, we have $\V(\F_{[0,1]}, ~ \B_{\ell_\infty, r}) = \mathcal{O}(t^{-d})$ and thus fail to certify.
}
\end{theorem}

\paragraph{Remark}
The condition 1) and 2)  in 
Theorem~\ref{thm: impossible linf} 
%The condition $\mathrm{mode}(\left\Vert \z\right\Vert _{\infty})=Cr$,
%$\left\Vert \z\right\Vert _{\infty}=\mathcal{O}_{p}(1)$  
 are used to ensure that the magnitude of the random perturbations generated by $\pizero$ is within a reasonable range such that the value of $\ff(\x)$ is not too small, in order to have a high accuracy  in the trade-off in \eqref{eq:objective2}. 
Note that the natural images are often contained in cube $[0,1]^{d}$. If $\norm{\z}_\infty$ is too large to exceed the region of natural images, 
%If the drawn samples are always out of %the region of natural images, which is often within $\norm{x}_\infty\leq 1$}, 
the accuracy will be obviously rather poor.
{
% \color{red}
Note that if we use variants of Gaussian distribution, we only need $||\z||_2/\sqrt{d}$ to be not too large.} 
%Therefore, 
% \red{(Why? do not see clear connection)}.
Theorem~\ref{thm: impossible linf} says that once
$\norm{\z}_\infty$ is in a reasonably small scale,   
the maximum distance term must be unreasonably large in high dimensions, yielding a vacuous lower bound.  
%However, once this condition is satisfied, our lower bound will becomes much smaller than a reasonable value, \emph{e.g.} $0.5$,  for large $d$.


% \paragraph{Practical Computation}
%This proposition shows we need a different smoothing distributionwhich can trade-off accuracy and robustness better than Gaussian distribution for $\ell_\infty$ case.We then propose the following distribution,
%$$\pi_{\boldsymbol{0}}(\z)&\propto\left\Vert \z\right\Vert _{\infty}^{-k}\exp\left(-\frac{\left\Vert \z\right\Vert _{2}^{2}}{2\sigma^{2}}\right).$$
 %Given a $\ell_\infty$ region $\|\d\|_\infty \leq r$,using Gaussian smoothingthe worst case $\d$ locates at $(r, r, \dots, r)$.Smoothing the classifier with our proposed distribution can also lead to a worst case located at $(r, r, \dots, r)$.Therefore, compared to the Gaussian distribution, the proposed distribution can lead to smaller $\D_+$.For a guaranteed lower bound, we prove the worst case $\{\d: \|\d\|_\infty \leq r \}$ with our proposed distribution.
 
\begin{figure*}

\begin{minipage}{0.4\textwidth}
% \vspace{-10pt}
%     \raisebox{2em}{\rotatebox{90}{\large Accuracy}}
    % \vspace{-40pt}
     \includegraphics[width=1.\textwidth]{fig/linf_example.pdf}\\
     \vspace{-10pt}
     \caption{
     For $\ell_\infty$ attacking, 
     the mixed norm distribution (right) 
     yields smaller TV distances (larger overlap areas), and hence higher robustness. 
     }
     %This figure shows the TV distance between $\pi_{\0}$ and $\pi_{\d}$. 
     %As shown above, the proposed distribution (right) 
     %can obtain smaller TV distance than Gaussian distribution (left). 
     %This fact indicates that our proposed distribution can yield more robustness while make less loss on accuracy.}
     \label{fig:c}
    %  \includegraphics[width=0.5\textwidth]{fig/cubeL2.pdf}\\
 %    \large{TV Distance (Robustness)}\\
%\end{tabular}
\end{minipage}
\hfill
\begin{minipage}{0.55\textwidth}
% \vspace{-60pt}
% \vspace{-40pt}
\begin{tabular}{c}
     \raisebox{2.0em}{\rotatebox{90}{ Accuracy}}
     \includegraphics[width=.9\textwidth]{fig/linf_tradeoff_3.pdf}\\
     { TV Distance (Robustness)}\\
\end{tabular}
\vspace{-5pt}
\caption{\small 
The Pareto frontier of 
accuracy and robustness (in the sense of \eqref{eq:objective2}) 
of the three smoothing families in \eqref{equ:L2smooth}, \eqref{equ:mixednormfamily}, and \eqref{eq:inf_inf_distribution} for $\ell_{\infty}$ attacking,  
when we search for the best parameters $(k,\sigma)$ for each of them. The mixed norm family \eqref{equ:mixednormfamily} yields the best trade-off than the other two. 
We assume $\ftrue(\vec x)=\mathbb{I}(\norm{\vec x}_2\leq r)$  and dimension $d=5$. The case when $\ftrue(\vec x)=\mathbb{I}(\norm{\vec x}_\infty\leq r)$ has similar result (not shown). 
}
\label{fig:linf_example}
\end{minipage}
\end{figure*}

 \paragraph{Empirical Justification}
 %To verify 
 We construct a simple toy example to verify the advantages of the mixed norm family \eqref{equ:mixednormfamily} overall the $\ell_2$ family in  \eqref{equ:L2smooth} and the $\ell_\infty$ family in  \eqref{eq:inf_inf_distribution}. 
 We assume that the true classifier is $\ftrue(\vv x) = \mathbb{I}(\norm{x}_2\leq r)$  in $r=0.65$, $d=5$ case
 and plot in Figure~\ref{fig:linf_example} the Pareto frontier of the accuracy and robustness terms in \eqref{eq:objective2} for the three families of smoothing distributions, as we search for the best combinations of parameters $(k, \sigma)$. 
 We can see that the mixed norm smoothing distribution clearly obtain the best trade-off on accuracy and robustness, and hence guarantees a tighter lower bound for certification.   
 

 %As shown in Figur~\ref{fig:linf_example},our proposed distribution can get better result than the distribution in \eqref{eq:inf_inf_distribution} and Gaussian distribution in the toy example. 


\paragraph{Computational Method}
In order to compute the lower bound when using the mixed norm family \eqref{equ:mixednormfamily}, 
we need to establish the closed form solution of the maximum distance term $\max_{\d \in \B}\D_{\F_{[0,1]}}(\lambda \pizero~||~ \pi_{\d})$ similar to Theorem~\ref{thm:opt_mu_l2}. 
%a variant of Theorem~\ref{thm:opt_mu_l2} 
%can be calculated using the same computational methods described. The only 
%The key is that distance term the $\max_{\d \in \B}\D_{\F_{[0,1]}}(\lambda \pizero~||~ \pi_{\d})$ yields a simple closed form due to symmetry, and the optimization on $\lambda\geq 0$ is one-dimensional and can be solved numerically efficiently. %because it is an . 
%it can still 
The following result shows that the optimal $\d$ is achieved at one vertex (the pointy points) of the $\ell_\infty$ ball. 
\begin{theorem} \label{thm:opt_mu_linf}
Consider the $\ell_{\infty}$ attack with  ${\B}_{\ell_\infty,r}=\left\{ \d:\left\Vert \d\right\Vert  _{\infty}\le r\right\}$ and the mixed norm smoothing distribution in \eqref{equ:mixednormfamily}
%$\pi_0$  $\pi_{\0}(\z)\propto\left\Vert \z\right\Vert _{\infty}^{-k}\exp\left(-\frac{\left\Vert \z\right\Vert _{2}^{2}}{2\sigma^{2}}\right)$ 
with $k\ge0$ and $\sigma>0$. 
Define $\d^{*} = [r,r,...,r]^\top$. 
We have for any $\lambda > 0$, 
$$
\mathbb{D}_{\mathcal{F}_{[0,1]}}\left(\lambda\pi_{\0}~\Vert~\pi_{\d^*}\right) = \max_{\delta\in\B}\mathbb{D}_{\mathcal{F}_{[0,1]}}\left(\lambda\pi_{\0}~\Vert~\pi_{\d}\right). 
$$
%where . 
%Consider the $\ell_{\infty}$ attack with $\boldsymbol{\mathcal{B}}=\left\{ \d:\left\Vert \d\right\Vert _{\infty}\le r\right\}$, given $\pi_{\0}(\z)\propto\left\Vert \z\right\Vert _{\infty}^{-k}\exp\left(-\frac{\left\Vert \z\right\Vert _{2}^{2}}{2\sigma^{2}}\right)$ for some $k\ge0$ and $\sigma>0$,
%we obtain $$\d^{*}=[r,r,...,r]^{\top}=\underset{\d\in\boldsymbol{\mathcal{B}}}{\arg\max}\ \mathbb{D}_{\mathcal{F}_{[0,1]}}\left(\lambda\pi_{\0}\parallel\pi_{\d}\right)$$for any $\lambda\ge0$. 
%Given a $d$ dimension perturbation $\|\d\|_\infty \leq r$ and a distribution $\pi_{\boldsymbol{0}}(\z)&\propto\left\Vert \z\right\Vert _\infty^{-k}\exp\left(-\frac{\left\Vert \z\right\Vert _{2}^{2}}{2\sigma_r^{2}}\right)$,
%$\d^* = \arg\max_{\d\in\mathcal{\B}}\D_+\left(\text{\ensuremath{\lambda}}\pi_{\0}(\cdot)\Vert \pi_{\d} (\cdot)\right)$ if and only if $|\d^*_i| = r$ for any $i \in \{1, \dots, d\}$.
\end{theorem}
The proof of Theorem \ref{thm:opt_mu_l2} and \ref{thm:opt_mu_linf} is non-trivial, thus we defer the details to Appendix \ref{sec: opt_mu_general_proof}.  With the optimal $\d^*$ found above, we can calculate the bound with similar Monte Carlo approximation outlined in Section~\ref{sec:L2}. 

